Compositional Sentence Representation from Character within Large Context Text

This paper describes a Hierarchical Composition Recurrent Network (HCRN) consisting of a 3-level hierarchy of compositional models: character, word and sentence. This model is designed to overcome two problems of representing a sentence on the basis of a constituent word sequence. The first is a data-sparsity problem in word embedding, and the other is a no usage of inter-sentence dependency. In the HCRN, word representations are built from characters, thus resolving the data-sparsity problem, and inter-sentence dependency is embedded into sentence representation at the level of sentence composition. We adopt a hierarchy-wise learning scheme in order to alleviate the optimization difficulties of learning deep hierarchical recurrent network in end-to-end fashion. The HCRN was quantitatively and qualitatively evaluated on a dialogue act classification task. Especially, sentence representations with an inter-sentence dependency are able to capture both implicit and explicit semantics of sentence, significantly improving performance. In the end, the HCRN achieved state-of-the-art performance with a test error rate of 22.7% for dialogue act classification on the SWBD-DAMSL database.

==> figure6_Effect_of_Hierarchical_Comp.tex <==

\begin{figure}[t]
 \centering
 \includegraphics[width=17cm]{figure6-effect_of_hier_comp.eps}
   \caption{Comparison of network to learn sentence representation from character. (a) With hierarchical composition  (b) Without hierarchical composition}
 \label{effect_of_hierarchical composition}
\end{figure}

